Encyclopedia Magneticum: Scaling Relations from Cosmic Dawn to Present Day

Galaxy and halo scaling relations, connecting a broad range of parameters, are well established from observations. The origin of many of these relations and their scatter is still a matter of debate. It remains a sizable challenge for models to simultaneously and self-consistently reproduce as many scaling relations as possible. We introduce the Magneticum Pathfinder hydrodynamical cosmological simulation suite, to date the suite that self-consistently covers the largest range in box volumes and resolutions. It is the only cosmological simulation suite that is tuned on the hot gas content of galaxy clusters instead of the stellar mass function. By assessing the successes and shortcomings of tuning to the hot gas component of galaxy clusters, we aim to further our understanding of the physical processes shaping the Universe. We analyze the importance of the hot and cold gas components for galaxy and structure evolution. We analyze 28 scaling relations, covering large-scale global parameters as well as internal properties for halos ranging from massive galaxy clusters down to galaxies, and show their predicted evolution from z=4 to z=0 in comparison with observations. These include the halo-to-stellar-mass and Kennicutt--Schmidt relations, the cosmic star formation rate density as well as the Fundamental Plane. Magneticum Pathfinder matches a remarkable number of the observed scaling relations from z=4 to z=0, including challenging relations like the number density of quiescent galaxies at cosmic dawn, the mass--size evolution, the mass--metallicity relation, the Magorrian relation, and the temperature--mass relation. We compile our data to allow for straightforward future comparisons. Galaxy properties and scaling relations arise naturally and the large scatter in observables at high redshift is crucial to distinguish the various galaxy formation models reproducing the z=0 relations.

==> style/linenoaa.tex <==
\NeedsTeXFormat{LaTeX2e}[2003/12/01]
\ProvidesPackage{linenoaa}[2023/03/12 v0.02]

\providecommand{\addto}[2]{%
  \ifx#1\@undefined
    \def#1{#2}%
  \else
    \ifx#1\relax
      \def#1{#2}%
    \else
      {\toks@\expandafter{#1#2}%
        \xdef#1{\the\toks@}}%
    \fi
  \fi
}

\newif\ifGPL@lineno@desactivate
\GPL@lineno@desactivatefalse

\DeclareOption{desactivate}{
	\providecommand{\@LN}{\@gobbletwo}
	\providecommand{\@LN@col}{\@gobble}
	\GPL@lineno@desactivatetrue	
}
\DeclareOption*{
	\PassOptionsToPackage{\CurrentOption}{lineno}
}
\ProcessOptions\relax

\ifGPL@lineno@desactivate
	\endinput
\fi

\RequirePackage[mathlines,switch]{lineno}[2005/11/02 v4.41]

\addto\maketitle{\linenumbers\relax}

\def\linenumberfont{\normalfont\scriptsize\sffamily}

\@namedef{eqnarray*}{\def\@eqncr{\nonumber\@seqncr}\linenomath\eqnarray}
\@namedef{endeqnarray*}{\nonumber\endeqnarray\endlinenomath}

\@ifpackageloaded{amsmath}{%
\renewenvironment{multline}{\linenomathNonumbers\start@multline\st@rredfalse}{%
	\iftagsleft@ \@xp\lendmultline@ \else \@xp\rendmultline@ \fi
	\endlinenomath\ignorespacesafterend}

\renewenvironment{multline*}{\linenomath\start@multline\st@rredtrue}{\endmultline\endlinenomath}


\renewenvironment{gather}{\linenomathNonumbers\start@gather\st@rredfalse}{%
  \math@cr \black@\totwidth@ \egroup
  $$\endlinenomath\ignorespacesafterend}

\renewenvironment{gather*}{\linenomath\start@gather\st@rredtrue}{\endgather\endlinenomath}

\renewenvironment{alignat}{\linenomathNonumbers\start@align\z@\st@rredfalse}{%
\endalign\endlinenomath}

\renewenvironment{alignat*}{\linenomath\start@align\z@\st@rredtrue}{\endalign\endlinenomath}

\renewenvironment{xalignat}{\linenomathNonumbers\start@align\@ne\st@rredfalse}{%
\endalign\endlinenomath}

\renewenvironment{xalignat*}{\linenomath\start@align\@ne\st@rredtrue}{\endalign\endlinenomath}

\renewenvironment{xxalignat}{\linenomath\start@align\tw@\st@rredtrue}{\endalign\endlinenomath}

\renewenvironment{align}{\linenomathNonumbers\start@align\@ne\st@rredfalse\m@ne}{%
  \math@cr \black@\totwidth@
  \egroup
  \ifingather@
    \restorealignstate@
    \egroup
    \nonumber
    \ifnum0=`{\fi\iffalse}\fi
  \else
    $$%
  \fi
  \endlinenomath
  \ignorespacesafterend}
  
\renewenvironment{align*}{\linenomath\start@align\@ne\st@rredtrue\m@ne}{\endalign\endlinenomath}

\renewenvironment{flalign}{\linenomathNonumbers\start@align\tw@\st@rredfalse\m@ne}{%
\endalign\endlinenomath}

\renewenvironment{flalign*}{\linenomath\start@align\tw@\st@rredtrue\m@ne}{\endalign\endlinenomath}

\renewenvironment{equation}{%
  \linenomathNonumbers\incr@eqnum
  \mathdisplay@push
  \st@rredfalse \global\@eqnswtrue
  \mathdisplay{equation}%
}{%
  \endmathdisplay{equation}%
  \mathdisplay@pop
  \endlinenomath
  \ignorespacesafterend}
    
\renewenvironment{equation*}{%
  \linenomath\mathdisplay@push
  \st@rredtrue \global\@eqnswfalse
  \mathdisplay{equation*}%
}{%
  \endmathdisplay{equation*}%
  \mathdisplay@pop
  \endlinenomath
  \ignorespacesafterend}}{%
\def\equation{\linenomathNonumbers$$\refstepcounter{equation}}
\def\endequation{\eqno \hbox{\@eqnnum}$$\endlinenomath\@ignoretrue}}

\@ifpackagewith{amsmath}{fleqn}{%
\renewenvironment{eqnarray}{%
    \stepcounter{equation}%
    \def\@currentlabel{\p@equation\theequation}%
    \global\@eqnswtrue\m@th
    \global\@eqcnt\z@
    \tabskip\mathindent
    \let\\=\@eqncr
    \setlength\abovedisplayskip{\topsep}%
    \ifvmode
      \addtolength\abovedisplayskip{\partopsep}%
    \fi
    \addtolength\abovedisplayskip{\parskip}%
    \setlength\belowdisplayskip{\abovedisplayskip}%
    \setlength\belowdisplayshortskip{\abovedisplayskip}%
    \setlength\abovedisplayshortskip{\abovedisplayskip}%
    \linenomathNonumbers$$\everycr{}\halign to\linewidth% $$
    \bgroup
      \hskip\@centering
      $\displaystyle\tabskip\z@skip{##}$\@eqnsel&%
      \global\@eqcnt\@ne \hskip \tw@\arraycolsep \hfil${##}$\hfil&%
      \global\@eqcnt\tw@ \hskip \tw@\arraycolsep
        $\displaystyle{##}$\hfil \tabskip\@centering&%
      \global\@eqcnt\thr@@
        \hb@xt@\z@\bgroup\hss##\egroup\tabskip\z@skip\cr}%
      {\@@eqncr
    \egroup
    \global\advance\c@equation\m@ne$$% $$
    \endlinenomath
    \@ignoretrue}}{}

